An Active Approach for Model Interpretation

Model interpretation, or explanation of a machine learning classifier, aims to extract generalizable knowledge from a trained classifier into a human-understandable format, for various purposes such as model assessment, debugging and trust. From a computaional viewpoint, it is formulated as approximating the target classifier using a simpler interpretable model, such as rule models like a decision set/list/tree. Often, this approximation is handled as standard supervised learning and the only difference is that the labels are provided by the target classifier instead of ground truth. This paradigm is particularly popular because there exists a variety of well-studied supervised algorithms for learning an interpretable classifier. However, we argue that this paradigm is suboptimal for it does not utilize the unique property of the model interpretation problem, that is, the ability to generate synthetic instances and query the target classifier for their labels. We call this the active-query property, suggesting that we should consider model interpretation from an active learning perspective. Following this insight, we argue that the active-query property should be employed when designing a model interpretation algorithm, and that the generation of synthetic instances should be integrated seamlessly with the algorithm that learns the model interpretation. In this paper, we demonstrate that by doing so, it is possible to achieve more faithful interpretation with simpler model complexity. As a technical contribution, we present an active algorithm Active Decision Set Induction (ADS) to learn a decision set, a set of if-else rules, for model interpretation. ADS performs a local search over the space of all decision sets. In every iteration, ADS computes confidence intervals for the value of the objective function of all local actions and utilizes active-query to determine the best one.

==> 0_abstract.tex <==
\begin{abstract}

\note{

Writing papers and managing projects are essential for conducting research.
A research paper describes the final outcomes, but can also help manage intermediate progress.
This document provides a template for writing papers and describes how to manage projects via drafts.

Start the abstract when you have some rough ideas, before they are forgotten amid your busy lives.
It does not need to be fancy, as long as you can understand your own writing later.
The eventual abstract should be the minimalist version of the entire paper, with key information outlined in the introduction.


}%note

(empty)

\end{abstract}


==> alg_sampling.tex <==
\begin{algorithm}
\caption{How to generate new synthetic instances. Given two decision set, we generate instances from the symmetric difference, i.e. the non-overlapping spaces of these two decision set.}
\label{sampling}
\begin{flushleft}
\textbf{INPUT:} $a^*,a'$ - two decision set \\
\textbf{Require}: $N_{batch}$ - the batch size of numbers of instances to generate and query each inner loop. $N_{MC}$ - the size of a Monte Carlo population, set to 1000 by default.
\end{flushleft}
\begin{algorithmic}[1]
\Procedure{GenerateSyntheticInstances}{$a^*,a',f$}

\State $d_1 \gets D_{a^*(S)} \setminus  D_{a'(S)} $
\State $d_2 \gets D_{a'(S)}  \setminus   D_{a^*(S)} $
% \State \Comment{Note that $d_1 \bigcup d_2$ is symmetric difference set}
\State $X' \gets \text{ActiveSampling}(d_1,f) \bigcup \text{ActiveSampling}(d_2,f) $
\State \Return $X'$
\EndProcedure

\Procedure{ActiveSampling}{$d$,$f$}
\State $X_{d} \gets \{ x| x \in d, x \in X \bigcup X'\},Y_{d} \gets f(X_{d})$  \Comment{ instances already covered in the region $d$}
\State $X'_{d} \gets X_{d},Y'_{d} \gets Y_{d} $
\For{ $ t = 1,\dots,N_{batch} $ }
\State $P \sim   { \{ \text{Uniform} (d) \} }_1^{N_{MC}}  $  \Comment{sample a random population}
\State $x_{\text{new}} \gets \mathop{\mathrm{argmax}}\limits_{x \in P} c \cdot \sigma(x) - |\hat{y} - 0.5|  $ \Comment{scoring function as mentioned in the paper}
\State $y_{\text{new}} \gets f(x_{\text{new}})$
\State $ X'_d \gets X'_d \bigcup x_{\text{new}} $
\State $ Y'_d \gets Y'_d \bigcup y_{\text{new}} $
% \State $X_{new} \gets X_{new} \bigcup x_{new}$
\EndFor
\State $ X'_d \gets X'_d \setminus X_d,  Y'_d \gets Y'_d \setminus Y_d$ \Comment{Return only new instances}
\State \Return $X'_d,Y'_d$
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> ccs.tex <==
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%
  
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371</concept_id>
<concept_desc>Computing methodologies~Computer graphics</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Computer graphics}


==> copyright.tex <==
\setcopyright{acmlicensed}



==> dart_throw_alg.tex <==
\begin{algorithm}
  \begin{algorithmic}[1]
    \REQUIRE sample domain $\domainsym$ with distance $\dist$ and conflict $\conflictdist$ measure
    \ENSURE output sample set $\sampleset$
    \STATE $\sampleset \assign \emptyset$
    \STATE $\failure \assign 0$ \pcomment{failure count}
    \WHILE{$\domainsym$ is not fully covered and $\failure$ not too high}
    \STATE $\sample \assign \funct{RandomSample}(\domainsym)$
    \IF{$\dist(\sample, \sampleprime) < \conflictdist(\sample, \sampleprime) \; \forall \sampleprime \in \sampleset$}
    \STATE $\sampleset \assign \sampleset \union \sample$ \pcomment{accept trial sample}
    \STATE $\failure \assign 0$
    \ELSE
    \STATE $\failure \assign \failure + 1$
    \ENDIF
    \ENDWHILE
    \RETURN{} $\sampleset$
  \end{algorithmic}
  \Caption{Dart throwing.}
  {%
This is an example of pseudo-code.
  }
  \label{alg:dart_throw}
\end{algorithm}




==> tog.tex <==
\acmJournal{TOG}
\acmYear{2017}
\acmVolume{36}
\acmNumber{4}
\acmArticle{1}
\acmMonth{7} % July
\acmDOI{}
\acmSubmissionID{papers\_0001}


